KU-DMIS at EHRSQL 2024:Generating SQL query via question templatization in EHR

Transforming natural language questions into SQL queries is crucial for precise data retrieval from electronic health record (EHR) databases. A significant challenge in this process is detecting and rejecting unanswerable questions that request information beyond the database's scope or exceed the system's capabilities. In this paper, we introduce a novel text-to-SQL framework that robustly handles out-of-domain questions and verifies the generated queries with query execution.Our framework begins by standardizing the structure of questions into a templated format. We use a powerful large language model (LLM), fine-tuned GPT-3.5 with detailed prompts involving the table schemas of the EHR database system. Our experimental results demonstrate the effectiveness of our framework on the EHRSQL-2024 benchmark benchmark, a shared task in the ClinicalNLP workshop. Although a straightforward fine-tuning of GPT shows promising results on the development set, it struggled with the out-of-domain questions in the test set. With our framework, we improve our system's adaptability and achieve competitive performances in the official leaderboard of the EHRSQL-2024 challenge.

==> tables/mimic_iv_table_info.tex <==

\begin{table*}[!htbp]
\centering
\begin{tabular}{@{}|l|p{10cm}|@{}}
\hline
\textbf{Table name} & \textbf{Description} \\
\hline
ADMISSIONS & Every unique hospitalization for each patient in the database (defines HADM\_ID). \\
\hline
CALLOUT & Information regarding when a patient was cleared for ICU discharge and when the patient was actually discharged. \\
\hline
CAREGIVERS & Every caregiver who has recorded data in the database (defines CGID). \\
\hline
CHARTEVENTS & All charted observations for patients. \\
\hline
CPTEVENTS & Procedures recorded as Current Procedural Terminology (CPT) codes. \\
\hline
D\_CPT & High level dictionary of Current Procedural Terminology (CPT) codes. \\
\hline
D\_ICD\_DIAGNOSES & Dictionary of International Statistical Classification of Diseases and Related Health Problems (ICD-9) codes relating to diagnoses. \\
\hline
D\_ICD\_PROCEDURES & Dictionary of International Statistical Classification of Diseases and Related Health Problems (ICD-9) codes relating to procedures. \\
\hline
D\_ITEMS & Dictionary of local codes ('ITEMID') appearing in the MIMIC database, except those that relate to laboratory tests. \\
\hline
D\_LABITEMS & Dictionary of local codes ('ITEMID') appearing in the MIMIC database that relate to laboratory tests. \\
\hline
DATETIMEEVENTS & All recorded observations which are dates, for example time of dialysis or insertion of lines. \\
\hline
DIAGNOSES\_ICD & Hospital assigned diagnoses, coded using the International Statistical Classification of Diseases and Related Health Problems (ICD) system. \\
\hline
DRGCODES & Diagnosis Related Groups (DRG), which are used by the hospital for billing purposes. \\
\hline
ICUSTAYS & Every unique ICU stay in the database (defines ICUSTAY\_ID). \\
\hline
INPUTEVENTS\_CV & Intake for patients monitored using the Philips CareVue system while in the ICU, e.g., intravenous medications, enteral feeding, etc. \\
\hline
INPUTEVENTS\_MV & Intake for patients monitored using the iMDSoft MetaVision system while in the ICU, e.g., intravenous medications, enteral feeding, etc. \\
\hline
OUTPUTEVENTS & Output information for patients while in the ICU. \\
\hline
LABEVENTS & Laboratory measurements for patients both within the hospital and in outpatient clinics. \\
\hline
MICROBIOLOGYEVENTS & Microbiology culture results and antibiotic sensitivities from the hospital database. \\
\hline
NOTEEVENTS & Deidentified notes, including nursing and physician notes, ECG reports, radiology reports, and discharge summaries. \\
\hline
PATIENTS & Every unique patient in the database (defines SUBJECT\_ID). \\
\hline
PRESCRIPTIONS & Medications ordered for a given patient. \\
\hline
PROCEDUREEVENTS\_MV & Patient procedures for the subset of patients who were monitored in the ICU using the iMDSoft MetaVision system. \\
\hline
PROCEDURES\_ICD & Patient procedures, coded using the International Statistical Classification of Diseases and Related Health Problems (ICD) system. \\
\hline
SERVICES & The clinical service under which a patient is registered. \\
\hline
TRANSFERS & Patient movement from bed to bed within the hospital, including ICU admission and discharge. \\
\hline
\end{tabular}
\caption{MIMIC-IV table information}
\label{tab:mimic_info}
\end{table*}


==> tables/null_detecting_dev.tex <==
\begin{table}
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ c|c|c }
\hline
\textbf{Model} & \textbf{\# of few-shot} & \textbf{RS(0)} \\ \hline\hline
GPT-3.5-turbo & 3 & 15.65 \\ \hline
Finetuned-GPT & - & 14.88 \\ \hline
GPT-4-turbo & 3 & 12.64 \\ \hline
GPT-4 & 3 & 9.97 \\ \hline
\end{tabular}
}
\caption{null detecting performance in dev set}
\label{tab:null_detectng_model_comparison}
\end{table}


==> tables/null_ratio_total.tex <==
\begin{table}
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ c|c c c }
\hline
\textbf{Model} & \textbf{train} & \textbf{dev} & \textbf{test} \\ \hline\hline
Null ratio & 8.95 & 19.95 & 19.97 \\ \hline
\end{tabular}
}
\caption{null ratio in train, dev, test set}
\label{tab:null_ratio}
\end{table}

